Computationally Relaxed Locally Decodable Codes, Revisited

We revisit computationally relaxed locally decodable codes (crLDCs) (Blocki et al., Trans. Inf. Theory '21) and give two new constructions. Our first construction is a Hamming crLDC that is conceptually simpler than prior constructions, leveraging digital signature schemes and an appropriately chosen Hamming code. Our second construction is an extension of our Hamming crLDC to handle insertion-deletion (InsDel) errors, yielding an InsDel crLDC. This extension crucially relies on the noisy binary search techniques of Block et al. (FSTTCS '20) to handle InsDel errors. Both crLDC constructions have binary codeword alphabets, are resilient to a constant fraction of Hamming and InsDel errors, respectively, and under suitable parameter choices have poly-logarithmic locality and encoding length linear in the message length and polynomial in the security parameter. These parameters compare favorably to prior constructions in the poly-logarithmic locality regime.

==> full-version/article-headers.tex <==
% !TeX root = main.tex
\usepackage{fullpage}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage[nameinlink,capitalize]{cleveref}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{fact}[theorem]{Fact}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

==> full-version/construction.tex <==
% !TeX root = main.tex
\section{Construction}
%In this section, we present our main theorem and our construction.
%\alex{Rework the theorem}


The rest of this section is dedicated describing our code construction and to proving \cref{thm:main}.
In \cref{sec:encoder}, we present our encoding algorithm $\Enc$; in \cref{sec:decoder}, we present our decoding algorithm $\Dec$.
Finally, in \cref{sec:main-proof}, we formally prove \cref{thm:main}.



\input{code-analysis}




%\newpage
%\input{scratch-work}


==> full-version/decoder.tex <==
\paragraph{The Decoder \texorpdfstring{$\Dec_\lambda$}{Dec\textsubscript{λ}}.}\label{sec:decoder}
We present the formal decoding algorithm $\Dec_\lambda$ in \cref{alg:decoder}. %; here, we give a high-level overview of the algorithm.
Let $x \in \bin{k}$ and $C = \Enc_\lambda(x)$, and suppose that $\tC \in \bin{n'}$ is a corrupt codeword such that $\ED(C, \tC) \leq \rho$ for some $n'$.
Given oracle access to $\tC$ and an index $i \in [k]$ as input, the decoder attempts to recover bit $x_i$ of the original message $x$.
Calling back to the encoding algorithm, bit $x_i$ resides in block $x\p{j}$ for $j$ satisfying $(j-1) \cdot r(\lambda) < i \leq j\cdot r(\lambda)$ (\cref{line:enc-block} of \cref{alg:encoder}).
Thus recovering $x_i$ is done by recovering block $x\p{j}$ from corrupt codeword $\tC$.
Assuming $\Dec_\lambda$ can recover $x\p{j}$, the decoder simply outputs $x_i = x\p{j}_{i^*}$ for $i^* = i - (j-1) \cdot r(\lambda)$; otherwise, our goal will be for $\Dec_\lambda$ to output $\bot$.

The decoder proceeds in two steps: first, the decoder attempts to recover the public key $\pk$ used to encode message $x$ as $C$ by running $\Enc_\lambda$; and second, the decoder attempts to recover some (possibly corrupt) block $\tildem = (\tildex \circ \tsigma \circ \tpk \circ \tildej)$.
The block $\tildem$ can then be parsed and verified using $\Verify_\pk$; that is, the decoder runs $\Verify_\pk( \tildex \circ j, \tsigma )$ and outputs $\tildex_{i^*}$ if $\Verify_\pk( \tildex \circ j, \tsigma ) = 1$ and outputs $\bot$ otherwise.
Note here that
\begin{enumerate*}[label=(\arabic*)]
	\item the public key $\pk$ recovered in the first step is not necessarily equal to string $\tpk$ parsed from $\tildem$ in the second step; and
	\item $\pk$ and desired block index $j$ are used to verify the string $\tildex$ rather than the parsed public key $\tpk$ and parsed index $\tildej$.
\end{enumerate*}

Towards the first goal of recovering the public key $\pk$, let $\omega \in \bbN$ be a parameter (to be determined later).
The decoder attempts to recover $\omega$ number of public keys, then take the majority of these recovered keys as the ``true'' public key $\pk$.
To do so, the decoder leverages the algorithm $\BlockDecode$.
On input $j \in [n']$, the algorithm $\BlockDecode$ queries the received word $\tC$ for a block to decode.
For example, if $\tC = C = \Enc_\lambda(x)$, then $\BlockDecode(1)$ would return $c\p{1}$ (as defined in \cref{eq:sz-enc} of \cref{alg:encoder}).
However, the algorithm $\BlockDecode$ is only guaranteed to return a correct block so long as the portion of $\tC$ it begins searching in is ``not too corrupt''.
This intuition is captured by the notion of a \emph{$\gamma$-good block}, which informally states that the edit distance between the uncorrupt block and the corrupt block is at most $\gamma$.
Then, so long as the number of $\gamma$-good blocks is large (for some constant $\gamma$), the \BlockDecode algorithm will succeed most of the time.
We formalize the notion of $\gamma$-good blocks in \cref{def:gamma-good} and the guarantees of \BlockDecode in \cref{lem:block-decode}.
This guarantees that with good probability (which depends on $\gamma$ and the value $\omega$), the public key recovered by the decoding algorithm (\cref{line:pk-majority}) is the correct public key used by the encoder; in particular, we can suitably choose $\omega$ such that $\pk^* = \pk$ with high probability via a Chernoff bound.

Conditioned on the decoder obtaining some public key $\pk^*$ in \cref{line:pk-majority}, the decoder proceeds in the next task of recovering the desired block $\tildem\p{j}$.
For this task, the decoder leverages the noisy-binary search algorithm \NBS. % given by \cref{lem:nbs}.
After running \NBS on input $j$ and obtaining some $\tildem\p{j}$, assuming that $\tildem\p{j} \neq \bot$, the decoder parses $\tildem\p{j}$ as the string $(\tildex\p{j} \circ \tsigma\p{j} \circ \tpk\p{j} \circ \tildej)$.
Then, as mentioned before, the decoder proceeds to verify that the signature $\tsigma\p{j}$ is a valid signature for the string $\tildex\p{j} \circ j$ using $\Verify$ and the recovered public key $\pk^*$.
It is important to again note that the index $j$ used in the verification may not be the same as $\tildej$, and that $\pk^*$ may not be the same as $\tpk\p{j}$.
One could alternatively choose for the decoder to output $\bot$ if either $j \neq \tildej$ or $\pk^* \neq \tpk\p{j}$; however, this would give the attacker an easy way to force the decoder to output $\bot$ on a large fraction of indices, something we want to avoid all together.
Finally, if the verification succeeds, the decoder outputs bit $\tildex\p{j}_{i^*}$ for $i^* = i - (j-1) \cdot r(\lambda)$.

\input{alg-decoder}

%\alex{need to put a note on what the block decode algorithm does here.}
%\alex{In overview, give an intuitive definition of what the block decoding algorithm does. E.g., as long as the block is not ``too corrupt'' (as will be explained later), and the index given to the algorithm is within a certain range, the algorithm always returns the correct string.}

==> full-version/encoder.tex <==
% !TeX root = main.tex


%Our construction is similar to that of Block \etal \cite{BBGKZ20}; in their case, the first encode each block $x\p{i}$ with a suitable Hamming \LDC.
%This yields a classical \LDC for InsDel errors.
%In our case, we forego the use of a Hamming \LDC for the use of signature schemes.
%While this prevents us from constructing a classical \LDC for InsDel errors, it gives us a computationally secure code and

==> full-version/lipics-headers.tex <==
% !TeX root = main.tex
\usepackage{thmtools}
\PassOptionsToPackage{nameinlink,capitalize}{cleveref}

==> full-version/old-code-analysis.tex <==
\alex{old analysis of \cref{item:rldc-fool} below here.}
Suppose towards contradiction that for adversary $\cA$, for all negligible functions $\eps_{\F}(\cdot)$, there exists a large enough $\lambda \in \bbN$ such that for $\tC = \cA(C)$, we have $\ED(C, \tC) \leq \rho$ and
%Suppose via contradiction that the adversary $\cA$ produces the codeword $\tC \in \bin{n'}$ such that $\ED(\tC,C) \leq \rho$ and
\begin{align*}
	\Pr\left[\Pr\left[ \exists i \in [k]~\colon~ D_i \in\{x_i, \bot\} \right] < p\right] > \eps_{\F}(\lambda).
\end{align*}
In other words, we have that
\begin{align*}
	\Pr\left[\Pr\left[ \exists i \in [k]~\colon~ D_i \not\in\{x_i, \bot\} \right] > 1-p\right] > \eps_{\F}(\lambda).
\end{align*}
We construct a new adversary $\cA'$ which breaks the security of the underlying signature scheme.
By \cref{def:sig} and \Cref{fig:sig-forge}, our adversary $\cA'$ is given $\pk$ as input and given oracle access to the function $\Sign_{\sk}(\cdot)$ for $(\pk, \sk) \gets \Gen(1^\lambda)$.
Given this input and this oracle, our adversary $\cA'$ does the following.
\begin{enumerate}
	\item $\cA'$ chooses any $x \in \bin{k}$.
	With $x$, our adversary $\cA'$ computes $C \in \bin{n}$ exactly as how the encoder $\Enc_\lambda$ of \cref{alg:encoder} would compute $C$, except with the following changes:
	\begin{itemize}
		\item $\cA'$ does not sample a public/private key pair (\cref{line:enc-key-sample}) \alex{Need to clarify exactly what the adversary does. Here, the adversary should embed the public key it is given into the constructed codeword.}; and
		\item $\cA'$ queries its oracle with $x\p{j} \circ j$ to compute $\sigma\p{j}$ of \cref{eq:sign}.
		\item \alex{$\cA'$ uses it's own $\pk$ when computing $y\p{i}$ for every $i$.}
	\end{itemize}
	
	\item $\cA'$ obtains corrupt codeword $\tC = \cA(C)$, where $\cA$ is the adversary against the \crLDC.
	
	\item For every index $i \in [k]$, $\cA'$ simulates $\Dec^{\tC}_\lambda(i)$ of \cref{alg:decoder} except with the following change:
	\begin{itemize}
		\item $\cA'$ skips the \textbf{foreach} loop of \cref{line:dec-for} and instead sets $\pk^* = \pk$ on \cref{line:pk-set}, where $\pk$ is the public key given to $\cA'$ as input.
	\end{itemize}
	During simulation, if $\tildex\p{j}$ parsed on \cref{line:tm-parse} satisfies 
	\begin{enumerate*}
		\item $\Verify_{\pk}(\tildex\p{j} \circ j, \tsigma\p{j}) = 1$; and
		\item $\tildex\p{j} \neq x\p{j}$,
	\end{enumerate*}
	then $\cA'$ halts simulation and outputs the pair $(\tildex, \tsigma)$, where $\tildex \defeq (\tildex\p{j} \circ j)$ and $\tsigma \defeq \tsigma\p{j}$.
\end{enumerate}

We now argue that our adversary $\cA'$ violates the security of the signature scheme $\Pi$ with non-negligible probability.
Clearly, our adversary $\cA'$ perfectly simulates the encoding algorithm $\Enc_\lambda$ by using its signature oracle $\Sign_{\sk}(\cdot)$.
Now if $Q$ is the set of oracle queries made by $\cA'$, then we have $Q = \{ (x\p{j}\circ j) \colon j \in [d] \}$, where $d = k/r(\lambda)$ and $x\p{j}$ are computed exactly as in \cref{line:enc-block} of \cref{alg:encoder} with message $x \in \bin{k}$ chosen by adversary $\cA'$.
Then $\cA'$ feeds codeword $C$ to adversary $\cA$ and obtains $\tC = \cA(C)$.
Since $C$ is identical to a codeword generated by $\Enc_\lambda$, we have that with probability greater than $\eps_{\F}(\lambda)$, we have that $\Pr[ \exists i \in [k]~\colon~ D_i \not\in\{x_i, \bot\} ] > 1-p$.
Now our adversary $\cA'$ simulates the decoder $\Dec^{\tC}(i)$ for every $i$.
Thus with probability greater than $1-p$, the decoder finds an index $i$ such that $D_i \not\in \{x_i, \bot\}$.
Suppose that this index $i$ resides in block $j^*$.
This implies that $\tildex\p{j^*} \neq x\p{j^*}$ and $\Verify_{\pk}(\tildex\p{j^*}\circ j, \tsigma\p{j^*}) = 1$.
Furthermore, this implies $\tildex\p{j^*} \not\in Q$.
Thus $(\tildex\p{j^*}, \tsigma\p{j^*})$ is a forgery.
This implies that 
\begin{align*}
	\Pr[\Sigforge_{\Pi, \cA}(\lambda) = 1] > (1-p)\cdot \eps_{\F}(\lambda).
\end{align*}
Thus for any $p \in (0,1)$, we have that $(1-p) \cdot \eps_{\F}(\lambda)$ is negligible in $\lambda$, and thus we arrive at our contradiction.
%	\alex{double check this statement with Jeremiah.}

Define random variable $X_\kappa$ for $\kappa \in [\omega]$ as
\begin{align*}
	X_\kappa = \begin{cases}
		1 & \BlockDecode^{\tC}(i_\kappa) = C\p{j_\kappa}\\
		0 & \text{otherwise}
	\end{cases},
\end{align*}
where $i_\kappa$ lies in block $j_\kappa$, and $C\p{j_\kappa}$ is the $j_\kappa$-th block of uncorrupt codeword $C = \Enc_\lambda(x)$.
Note that $i_\kappa$ is sampled uniformly at random, and that runs of $\BlockDecode$ are independent of one another.
Thus for any $\kappa \in [\omega]$, we have that
\begin{align*}
	\Pr[X_\kappa = 1] &= \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ]\\
	&= \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-good} ] \cdot \Pr[j_\kappa \text{ is $\gamma$-good}] \\
	&+ \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-bad} ] \cdot \Pr[j_\kappa \text{ is $\gamma$-bad}] \\
	&\geq \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-good} ] \cdot \Pr[j_\kappa \text{ is $\gamma$-good}].
\end{align*}
By \cref{lem:block-decode}, we know that
\begin{align*}
	\Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-good} ] \geq 1-\gamma.
\end{align*}
Now for $\Pr[j_\kappa \text{ is $\gamma$-good}]$, we utilize \cref{lem:gamma-block-bounds} and the fact that $i_\kappa \getsr [n']$.
\begin{align*}
	\Pr[j_\kappa \text{ is $\gamma$-good}] &= \Pr[i_\kappa \in \text{ any $\gamma$-good block}] \geq \frac{ (\beta-\alpha\cdot \gamma) \cdot \tau \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right)\cdot d }{n'}\\
	&= \frac{(\beta-\alpha\cdot \gamma) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right) \cdot \left(\frac{n}{\beta}\right)}{n'} \geq \frac{(\beta-\alpha\cdot \gamma) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right) \cdot \left(\frac{n}{\beta}\right)}{(1+\rho)\cdot n}\\
	&=\left(\frac{\beta - \alpha \cdot \gamma}{(1+\rho) \cdot \beta}\right) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right)
\end{align*}
Thus we have that
\begin{align*}
	\Pr[X_\kappa = 1] \geq (1-\gamma) \cdot \left(\frac{\beta - \alpha \cdot \gamma}{(1+\rho) \cdot \beta}\right) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right)
\end{align*}
where the right hand side is $> 1/2$ for suitably chosen constants $\gamma$ and $\alpha$.
Thus if $q \defeq \Pr[X_\kappa = 1]$, then we have that $q > 1/2$.
Let $\eta \defeq \eta(n)$ be a suitably chosen such that $\omega \geq \log(1/\eta) \cdot (2q) / (q-1/2)^2 = \Theta(\log^{1+\epsilon}(n))$ for small $\epsilon > 0$.
Then by Chernoff bound and the fact that $X_\kappa$ are all i.i.d. and independent, we have that
\begin{align*}
	\Pr\left[ \sum_{\kappa \in [\omega]} X_\kappa > \frac{\omega}{2} \right] \geq 1 - e^{\frac{-1}{2p} \cdot \omega \cdot (p-1/2)^2} \geq 1-\eta.
\end{align*}
This implies that 
\begin{align*}
	\Pr[\pk^* = \pk] = \Pr[\pred{majority}(\pk\p{i_1},\dotsc, \pk\p{i_\omega}) = \pk] \geq 1-\eta.
\end{align*}
%	Moreover, as $\omega = \Theta(\log^3(n))$, recovering $\pk^*$ has query complexity

==> full-version/overview.tex <==
% !TeX root = main.tex
\subsection{Technical Overview}\label{sec:overview}
%In this work, we construct computationally relaxed locally decodable codes (or \crLDC{}s in short) that are resilient to adversarial insertion-deletion errors made by a computationally bounded channel (\ie, our channels are assumed to be probabilistic polynomial time, or PPT in short).
%We begin by formally defining such codes that are relevant to our model.
%\begin{definition}[Computationally Relaxed Locally Decodable Codes]\label{def:crldc}
%	Let $\cC = \{ C_\lambda[ K, k, q_1, q_2 ] \}_{\lambda \in \bbN}$ be a family of coding schemes with encoding algorithms $\{ \Enc_\lambda \colon \Sigma_1 \rightarrow \Sigma_2 \}_{\lambda \in \bbN}$ where $|\Sigma_i| = q_i$.
%	We say $\cC$ is a \emph{$(\ell, \rho, p, \delta, \dist)$-computationally relaxed locally decodable code} (\crLDC) if there exists a family of randomized oracle decoding algorithms $\{ \Dec_\lambda \colon \{1,\dotsc, k\} \rightarrow \Sigma_1 \}_{\lambda \in \bbN}$ satisfying the following properties.
%	\begin{enumerate}
%		\item For all $\lambda \in \bbN$ and any word $\tildey \in \Sigma_2^*$, the algorithm $\Dec^{\tildey}_\lambda(i)$ makes at most $\ell$ queries to $\tildey$ for any $i \in [k]$;
%		
%		\item For all $\lambda \in \bbN$ and any message $x \in \Sigma_1^k$, we have that $\Pr[ \Dec_\lambda^{\Enc_\lambda(x)}(i) = x_i ] = 1$ for all $i \in [k]$;\label{item:rldc-correct}
%		
%		\item Define binary predicate $\Fool(y', \rho, p, x, y, \lambda) = 1$ iff
%		\begin{enumerate}
%			\item $\dist(y,y')\leq \rho$; and
%			\item $\exists i \in [k]$ such that $\Pr[\Dec_\lambda^{y'}(i) \in \{x_i, \bot\}] < p$,
%		\end{enumerate}
%		where the probability is taken over the random coins of $\Dec_\lambda$; otherwise $\Fool(y', \rho, p, x ,y) = 0$.
%		We require that for all PPT adversaries $\cA$ there exists a negligible function $\eps_{\F}(\cdot)$ such that for all $\lambda \in \bbN$ and all $x \in \Sigma_1^k$, we have
%		\begin{align*}
%			\Pr[ \Fool(\cA(y), \rho, p, x, y, \lambda) = 1 ] \leq \eps_{\F}(\lambda),
%		\end{align*}
%		where the probability is taken over the random coins of $\cA$ and $y = \Enc_\lambda(x)$.\label{item:rldc-fool}
%		
%		\item Define binary predicate $\Limit(y', \rho, \delta, x, y, \lambda) = 1$ if and only if the following hold:
%		\begin{enumerate}
%			\item $\dist(y,y') \leq \rho$; and
%			\item $|\Good(y')| < \delta \cdot k$, where $$\Good(y') \defeq \{ i \in [k] \colon \Pr[\Dec_\lambda^{y'}(i) = x_i] > 2/3 \},$$
%		\end{enumerate}
%		where the probability is taken over the random coins of $\Dec_\lambda$; otherwise $\Limit(y', \rho, \delta, x, y, \lambda) = 0$.
%		We require that for all adversaries PPT adversaries $\cA$ there exists a negligible function $\eps_{\Lim}(\cdot)$ such that for all $\lambda \in \bbN$ and all $x \in \Sigma_1^k$, we have
%		\begin{align*}
%			\Pr[\Limit(\cA(y), \rho, \delta, x, y, \lambda) = 1] \leq \eps_{\Lim}(\lambda),
%		\end{align*}
%		where the probability is taken over the random coins of $\cA$ and $y = \Enc_\lambda(x)$.\label{item:rldc-limit}
%	\end{enumerate}
%	If $\dist$ is the normalized Hamming distance $\HAM$, we say the code is a \emph{Hamming \crLDC}; if $\dist$ is the normalized edit distance $\ED$, we say the code is a \emph{InsDel \crLDC}.
%	Here, $\ell$ is the \emph{locality} of $\cC$, $\rho$ is the \emph{error-tolerance} of $\cC$, and $k/K$ is the \emph{rate} of $\cC$. 
%	If $q_2 = 2$, we say that $\cC$ is a family of \emph{binary \crLDC{}s}.
%	For convenience, if $q_1 = q_2$, we simply write $C_\lambda[K,k,q_1]$.
%\end{definition}
%Our definition captures the notion of asymptotic security when interacting with arbitrary PPT adversarial channels $\cA$.
%We differ from the \crLDC definition of Blocki \etal \cite{..} in two key ways.
%First, \cite{..} defines their codes with respect to a public parameter generation function $\Gen(1^\lambda)$ which on input security parameter $\lambda$ in unary generates some public seed $s\in\bin{*}$ that is fixed once and for all. 
%In our case, the security parameter $\lambda$ is captured by a family of codes $\cC = \{C_\lambda\}_{\lambda \in \bbN}$, calling back to circuit family definitions.
%Second, we require our codes to satisfy a stronger notion of $\Fool$.
%\cite{..} defines the predicate $\Fool$ analogously to \cref{def:crldc}, except they allow an adversary to choose the index $i \in [k]$ such that $\Pr[\Dec_\lambda^{y'}(i) \in \{x_i,\bot\}] <p$.
%In our case, the adversary wins simply if there exists any such index $i \in [k]$, even if that index was not an index targeted by the adversary.

















%We construct computationally relaxed locally decodable codes (\crLDC{}s) that are resilient against insertion-deletion errors by adapting the so-called ``Hamming-to-InsDel'' compiler of Block \etal \cite{..}.
%Intuitively, this compiler extends the ideas of \emph{concatenation codes} to the insertion-deletion setting.
%In standard concatenation codes, there are two separate Hamming codes: the inner code $\Cin = (\Encin, \Decin)$ and the outer code $\Cout = (\Encout, \Decout)$.
%Then the concatenation code $C = (\Enc,\Dec)$ operates as follows.
%For any message $x$, $\Enc(x)$ first computes $c = \Encout(x)$.
%Next, the codeword $c$ is divided into some number $d$ of blocks $c = c\p{1}\circ \cdots \circ c\p{d}$.
%Then, for each block $i \in \{1,2,\dotsc, d\}$, a new block $C\p{i} = \Encin(c\p{i})$ is computed.
%The final codeword is the concatenation of these new blocks; \ie, $C = C\p{1}\circ \cdots \circ C\p{d} =  \Enc(x)$.
%In the case that both $\Cin$ and $\Cout$ are Hamming codes, the deocding algorithm is simple: for a corrupt codeword $C'$, simply partition $C'$ into $d$ blocks, run $\Decin$ on each block and concatenate all the results, then run $\Decout$ on this new string and output according to $\Decout$.
%
%The case for when 


%\alex{This is garbage, come back and rewrite}
%Our construction of a computationally relaxed locally decodable code (\crLDC) that is resilient against insertion-deletion errors borrows from the well-known techniques of concatenation codes \cite{..}.
%Briefly, a concatenation code is composed of two error-correcting codes, an inner code $\Cin = (\Encin, \Decin)$ and an outer code $\Cout = (\Encout,\Decout)$.
%The encoding algorithm of a concatenation code first takes a message $x$ and computes a codeword $c = \Encout(x)$.
%The codeword $c$ is then partitioned into some number, say $d$, blocks $c = c\p{1} \circ \cdots \circ c\p{d}$, and each block $c\p{i}$ is then encoded as $C\p{i} = \Encin(c\p{i})$ for every $i \in [d]$.
%The final codeword $C$ is a concatenation of all blocks $C\p{1} \circ \cdots \circ C\p{d}$.
%
%In standard applications of concatenation codes, both the inner and outer codes are \emph{Hamming} codes; in our case, we differ in two key ways.
%First, we use \emph{digital signatures} in place of an outer code; and second, our inner code is an \emph{insertion-deletion code}.
%The former allows us concrete efficiency gains over the use of a standard Hamming code at the cost of assuming a computationally bounded adversary, while the latter gives us resilience to a broader class of errors.

==> full-version/scratch-work.tex <==
% !TeX root = main.tex
\section{Scratch Work}

Let $E_i \defeq \Pr[\Dec^{\tC}(i) \in \{x_i, \bot\}] \geq p$.
Need to show that $\Pr[\exists i \in [n] \colon \overline{E}_i] \leq \eps$; or, equivalently, $\Pr[\forall i \in [n] \colon E_i] \geq 1 - \eps$.
Let $i \in [k]$ be arbitrary.
We first provide an upper bound on $\Pr[\Dec^{\tC}(i) \in \{x_i, \bot\}]$.

First we have that
\begin{align*}
	\Pr[\Dec^{\tC}(i) \in \{x_i, \bot\}] = \Pr[ \Dec^{\tC}(i) = x_i ] + \Pr[\Dec^{\tC}(i) = \bot].
\end{align*}
This follows since the event that the decoder outputs $\bot$ is mutually exclusive from the event that the decoder outputs any other symbol.
We now bound the above probability by upper bounding each of the events.

Let $D_i(\bot)$ be the event that $\Dec^{\tC}(i) = \bot$. 
Then we observe that
\begin{align}
	\Pr[D_i(\bot)] &= \Pr[\pk^* = \bot]\label{eq:pk-bot}\\
	&+ \Pr[\tildem\p{j} = \bot ~|~ \pk^* \neq \bot] \cdot \Pr[\pk^* \neq \bot]\label{eq:mj-bot}\\
	&+ \Pr[ \Verify_{\pk^*}(x\p{j} \circ j, \tsigma\p{j}) = 0 ~|~ \tildem\p{j} \neq \bot \band  \pk^* \neq \bot ] \cdot \Pr[ \tildem\p{j} \neq \bot \band  \pk^* \neq \bot ]\label{eq:ver-bot}
\end{align}
We lower bound each of the terms in the above equation.
First consider \cref{eq:pk-bot}.
To analyze this probability, we turn to the simpler task of analyzing $\Pr[\pk^* = \pk]$; that is, the probability that the decoder recovers the correct public key.
Define random variable $X_\kappa$ for $\kappa \in [\omega]$ as
\begin{align*}
	X_\kappa = \begin{cases}
		1 & \BlockDecode^{\tC}(i_\kappa) = C\p{j_\kappa}\\
		0 & \text{otherwise}
	\end{cases},
\end{align*}
where $i_\kappa$ lies in block $j_\kappa$, and $C\p{j_\kappa}$ is the $j_\kappa$-th block of uncorrupt codeword $C = \Enc(x, 1^\lambda)$.
Note that $i_\kappa$ is sampled uniformly at random, and that runs of $\BlockDecode$ are independent of one another.
Thus for any $\kappa \in [\omega]$, we have that
\begin{align*}
	\Pr[X_\kappa = 1] &= \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ]\\
	&= \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-good} ] \cdot \Pr[j_\kappa \text{ is $\gamma$-good}] \\
	&+ \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-bad} ] \cdot \Pr[j_\kappa \text{ is $\gamma$-bad}] \\
	&\geq \Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-good} ] \cdot \Pr[j_\kappa \text{ is $\gamma$-good}].
\end{align*}
By \cref{lem:block-decode}, we know that
\begin{align*}
	\Pr[ \BlockDecode^{\tC} = C\p{j_\kappa} ~|~ j_\kappa \text{ is $\gamma$-good} ] \geq 1-\gamma.
\end{align*}
Now for $\Pr[j_\kappa \text{ is $\gamma$-good}]$, we utilize \cref{lem:bad-block-frac,lem:good-block-bound} and the fact that $i_\kappa \getsr [n']$.
\begin{align*}
	\Pr[j_\kappa \text{ is $\gamma$-good}] &= \Pr[i_\kappa \in \text{ any $\gamma$-good block}] \geq \frac{ (\beta-\alpha\cdot \gamma) \cdot \tau \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right)\cdot d }{n'}\\
	&= \frac{(\beta-\alpha\cdot \gamma) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right) \cdot \left(\frac{n}{\beta}\right)}{n'} \geq \frac{(\beta-\alpha\cdot \gamma) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right) \cdot \left(\frac{n}{\beta}\right)}{(1+\rho)\cdot n}\\
	&=\left(\frac{\beta - \alpha \cdot \gamma}{(1+\rho) \cdot \beta}\right) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right)
\end{align*}
Thus we have that
\begin{align*}
	\Pr[X_\kappa = 1] \geq (1-\gamma) \cdot \left(\frac{\beta - \alpha \cdot \gamma}{(1+\rho) \cdot \beta}\right) \cdot \left(1 - \frac{2\cdot \beta \cdot \rho}{\alpha \cdot \gamma} \right)
\end{align*}
where the right hand side is $> 1/2$ for suitably chosen constants $\gamma$ and $\alpha$.
Thus if $p \defeq \Pr[X_\kappa = 1]$, then we have that $p > 1/2$.
Let $\eta > 0$ be a suitable constant and let $\omega \geq \log(1/\eta) \cdot (2p) / (p-1/2)^2$ be a constant.
Then by Chernoff bound and the fact that $X_\kappa$ are all i.i.d. and independent, we have that
\begin{align*}
	\Pr\left[ \sum_{\kappa \in [\omega]} X_\kappa > \frac{\omega}{2} \right] \geq 1-\eta.
\end{align*}
This implies that 
\begin{align*}
	\Pr[\pred{majority}(\pk\p{i_1},\dotsc, \pk\p{i_\omega}) = \pk] \geq 1 - e^{\frac{-1}{2p} \cdot \omega \cdot (p-1/2)^2} \geq 1-\eta.
\end{align*}
Thus we have that
\begin{align*}
	\Pr[\pk^* = \pk] \geq 1 - e^{\frac{-1}{2p} \cdot \omega \cdot (p-1/2)^2} \geq 1-\eta,
\end{align*}
and finally
\begin{align*}
	\Pr[\pk^* = \bot] \leq \Pr[\pk^* \neq \pk] = 1-\Pr[\pk^* = \pk] \leq e^{\frac{-1}{2p} \cdot \omega \cdot (p-1/2)^2} \leq \eta.
\end{align*}

Next we analyze \cref{eq:mj-bot}.

%
%\mbox{}\\
%\alex{Ignore below for now}
%By definition, we have that
%\begin{align*}
%	\pk^* = \bot \iff \pred{majority}(\pk\p{i_1},\dotsc, \pk\p{i_{\omega}}) = \bot.
%\end{align*}
%For $\kappa \in [\omega]$, define random variable
%\begin{align*}
%	X_\kappa = \begin{cases}
%		1 & \BlockDecode^{\tC}(i_\kappa) = \bot\\
%		0 & \text{otherwise}
%	\end{cases}.
%\end{align*}
%Let $X \defeq \sum\limits_{\kappa \in [\omega]} X_\kappa$ and without loss of generality assume that $\omega$ is odd.
%Then we have that
%\begin{align*}
%	\Pr[\pk^* = \bot] = \Pr\left[ X \geq  \frac{\omega+1}{2}\right].
%\end{align*}
%We now analyze $\Pr[X_\kappa = 1]$ for any $\kappa \in [\omega]$.
%By the algorithm $\BlockDecode$, we have that
%\begin{align*}
%	\Pr[X_\kappa = 1] &= \Pr[\BlockDecode^{\tC}(i_{\kappa})= \bot]\\
%	&= \Pr[\BlockDecode^{\tC}(i_{\kappa})= \bot | i_{\kappa} \text{ is in a $\gamma$-good block}] \cdot \Pr[i_{\kappa} \text{ is in a $\gamma$-good block}]\\
%	&+ \Pr[\BlockDecode^{\tC}(i_{\kappa})= \bot | i_{\kappa} \text{ is in a $\gamma$-bad block}] \cdot \Pr[i_{\kappa} \text{ is in a $\gamma$-bad block}]
%\end{align*}
%
%By \cref{lem:block-decode} we have that $\Pr[\BlockDecode^{\tC}(i_{\kappa})= \bot | i_{\kappa} \text{ is in a $\gamma$-good block}] \leq \gamma$.
%We need the following bound as well.
%%\begin{lemma}[\cite{BBGKZ20}]\label{lem:good-block-bound}
%%	For any $\gamma$-good block $j$, we have that $(\beta - \alpha\gamma) \cdot \tau \leq |\phi_0^{-1}(j)| \leq (\beta + \alpha\gamma) \cdot \tau$, where $\tau = |x\p{j} \circ \sigma\p{j} \circ \pk \circ j| = 2\log(k) + \lambda^c$.
%%\end{lemma}
%Since \cref{lem:bad-block-frac} only gives us an upper bound on the total fraction of $\gamma$-bad blocks, and the total fraction of $\gamma$-good blocks can be at most $1$, the best bound of $\Pr[i_{\kappa} \text{ is in a $\gamma$-good block}]$ we can hope for is upper bounding by $1$.
%Similarly, \cref{lem:block-decode} doesn't tell us the probability that $\BlockDecode$ outputs $\bot$ if $i_\kappa$ is in a $\gamma$-bad block; thus the best we can hope for is $\Pr[\BlockDecode^{\tC}(i_{\kappa})= \bot | i_{\kappa} \text{ is in a $\gamma$-bad block}] \leq 1$.
%Then by \cref{lem:bad-block-frac,lem:good-block-bound}, we have that \alex{import derivation from iPad}
%\begin{align*}
%	\Pr[i_{\kappa} \text{ is in a $\gamma$-bad block}] \leq 1 - \frac{\left(1 - \frac{2\beta\rho}{\alpha\gamma}\right) \cdot (\beta-\alpha\gamma)}{(1+\rho)\cdot \beta}
%\end{align*}
%Thus we have that
%\begin{align*}
%	\Pr[X_\kappa = 1] \leq \gamma + 1 - \frac{\left(1 - \frac{2\beta\rho}{\alpha\gamma}\right) \cdot (\beta-\alpha\gamma)}{(1+\rho)\cdot \beta}.
%\end{align*}
%Then we have by Markov's inequality
%\begin{align*}
%	\Pr[\pk^* = \bot] = \Pr\left[ X \geq \frac{\omega+1}{2} \right] \leq \left(\frac{2\cdot \omega}{\omega + 1}\right) \cdot \left(\gamma + 1 - \frac{\left(1 - \frac{2\beta\rho}{\alpha\gamma}\right) \cdot (\beta-\alpha\gamma)}{(1+\rho)\cdot \beta}\right).
%\end{align*}

==> full-version/security.tex <==
\paragraph{Proof of Security Overview.}\label{sec:security}
The main technical challenge of our construction is showing our construction satisfies \cref{item:rldc-fool,item:rldc-limit} of \cref{def:crldc}.
We present the formal proof of security in \cref{sec:main-proof} and give a high level overview in the remainder of this section.

Towards analyzing \cref{item:rldc-fool}, we appeal to the security of the signature scheme $\Pi$.
Supposing that there exists an adversary $\cA$ which violates \cref{item:rldc-fool}, then we can construct an adversary $\cA'$ which violates the security of the scheme $\Pi$.
This adversary $\cA'$ operates as follows: given input $\pk$ and oracle $\Sign_{\sk}$, the adversary $\cA'$ chooses an arbitrary message $x\in \bin{k}$ and simply copies what the encoder $\Enc_\lambda$ does, except $\cA'$ does not sample a public/private key pair and instead 
\begin{enumerate*}[label*=(\arabic*)]
	\item uses its input $\pk$ as the public key; and
	\item uses its oracle $\Sign_{\sk}$ to compute the signatures $\sigma\p{j}$.
\end{enumerate*}
So $\cA'$ identically computes $C = \Enc_\lambda(x)$ as $\Enc_\lambda$ would have conditioned on generating $(\pk,\sk)$.
The adversary then obtain $\tC$ from adversary $\cA(C)$.
Since $\cA$ violates \cref{item:rldc-fool}, with non-negligible probability there exists an index $i \in [k]$ such that the probability $\Pr[\Dec_\lambda^{\tC}(i) \in \{x_i, \bot\}] < p$, or equivalently $\Pr[\Dec_\lambda^{\tC}(i) \not\in \{x_i, \bot\}] > 1-p$. 
At this point $\cA'$ simply runs the noisy-binary search algorithm \NBS for every block $j \in \{1,\dotsc, d\}$ until it obtains a corrupt block $\tildem\p{j} = (\tildex\p{j} \circ \tsigma\p{j} \circ \tpk \circ \tildej)$ such that $(\tildex\p{j} \circ j, \tsigma\p{j})$ is a pair that violates the security of the signature scheme $\Pi$.
Thus $\cA'$ violates the security of $\Pi$ with non-negligible probability, which contradicts our assumption on the signature scheme.

Towards analyzing \cref{item:rldc-limit}, we appeal to the properties of both \BlockDecode and \NBS, along with the fact that the number of $\gamma$-good blocks is large.
First, since the number of $\gamma$-good blocks is large, if we sample a sufficiently large number $\omega$ of indices to run $\BlockDecode$ on, then with high probability (via a Chernoff bound) the recovered public key $\pk^*$ will be equal to the true public key $\pk$.
Next, we leverage the guarantees of the algorithm \NBS.
That is, except with negligible probability the algorithm \NBS recovers a $\gamma$-good block $j$ with good probability.
This implies that except with negligible probability, $\tildem\p{j}$ will be the correct value if $j$ is $\gamma$-good.
Finally, since the number of $\gamma$-good blocks is large, we argue that except with negligible probability, the number of indices $i \in \{1,\dotsc, k\}$ for which $\Dec^{\tC}_\lambda(i) = x_i$ is large (proportional to the number of $\gamma$-good blocks).
Note that this bound holds \emph{for any} $\tC$ satisfying $\ED(C,\tC) \leq \rho$ for $C = \Enc_\lambda(x)$.
